Trajectory Consistency for One-Step Generation on Euler Mean Flows

We propose \emph{Euler Mean Flows (EMF)}, a flow-based generative framework for one-step and few-step generation that enforces long-range trajectory consistency with minimal sampling cost. The key idea of EMF is to replace the trajectory consistency constraint, which is difficult to supervise and optimize over long time scales, with a principled linear surrogate that enables direct data supervision for long-horizon flow-map compositions. We derive this approximation from the semigroup formulation of flow-based models and show that, under mild regularity assumptions, it faithfully approximates the original consistency objective while being substantially easier to optimize. This formulation leads to a unified, JVP-free training framework that supports both $u$-prediction and $x_1$-prediction variants, avoiding explicit Jacobian computations and significantly reducing memory and computational overhead. Experiments on image synthesis, particle-based geometry generation, and functional generation demonstrate improved optimization stability and sample quality under fixed sampling budgets, together with approximately $50\%$ reductions in training time and memory consumption compared to existing one-step methods for image generation.

==> bo_notes.tex <==
- 不确定能不能用dynamics这个词，它在生成模型里有什么特别含义吗？我理解生成模型里并没有力这个概念，可以看看以前的文章有没有用这个词的

- related work 每段一个标题

- shorten related work，删掉一些单纯的评论性的文字（比如第一段最后两句），看着像AI写的

- mild condition 出现了好几次，最好可以换成比较具体的描述

- 可以把最重要的式子框出来


